Newton-Okounkov bodies of chemical reaction systems

Despite their noted potential in polynomial-system solving, there are few concrete examples of Newton-Okounkov bodies arising from applications. Accordingly, in this paper, we introduce a new application of Newton-Okounkov body theory to the study of chemical reaction networks, and compute several examples. An important invariant of a chemical reaction network is its maximum number of positive steady states, which is realized as the maximum number of positive real roots of a parametrized polynomial system. Here, we introduce a new upper bound on this number, namely the `Newton-Okounkov body bound' of a chemical reaction network. Through explicit examples, we show that the Newton-Okounkov body bound of a network gives a good upper bound on its maximum number of positive steady states. We also compare this Newton-Okounkov body bound to a related upper bound, namely the mixed volume of a chemical reaction network, and find that it often achieves better bounds.

==> Images/BCY_NOB.tex <==
        \begin{tikzpicture}
        \node[] (1) at (0,0){}; %{$(2,2)$};
        \node[] (2) at (2,0){}; %{$(3,2)$};
        \node[] (3) at (2,2){}; %{$(3,3)$};
        \node[] (4) at (0,2){}; %{$(2,3)$};
        \node[] (nob) at (1,1) {{\Huge $\Delta$}};
        \draw[fill = black] (0,0) circle (2.5pt) node[anchor=north] {$(2,2)$};
        \draw[fill = black] (2,0) circle (2.5pt) node[anchor=north] {$(3,2)$};
        \draw[fill = black] (2,2) circle (2.5pt) node[anchor=south] {$(3,3)$};
        \draw[fill = black] (0,2) circle (2.5pt) node[anchor=south] {$(2,3)$};
        \filldraw[line width=2pt,color=black,fill=black] (1) -- (2) -- (3) -- (4) -- (1) -- cycle;
        \end{tikzpicture}

==> m2-nob.tex <==
\section{Supporting computations}\label{app:nob}

We provide the {\tt Macaulay2} input code to compute the volume of the Newton-Okounkov body and augMV for the chemical reaction system from Example~\ref{ex:polly-paper-ex-4.1}. 

% --- Example 7.5.1
\begin{verbatim}
--- xdot = p1(p2-p3)
--- ydot = p1(p4-p5)

restart
needsPackage "SubalgebraBases"
needsPackage "Polyhedra" 
R = QQ[x,y];
p1 = x^2*y^2 + x^2 + y^2 + 1 -5*x*y;
p2 = 1;
p3 = x*y;
p4 = x;
p5 = y;

-- compute volume of Newton-Okounkov body
G = {p1*p2, p1*p3, p1*p4, p1*p5} --choose to be generating set G
SAGBIbasis = sagbi(matrix {G})   
NObody = convexHull(transpose matrix (flatten for i in G 
                                    list exponents leadTerm(i)))
volumeNObody = (numgens R)!*volume(NObody)

-- compute mixed volume of system (augMV)
needsPackage("PHCpack")
R = CC[x,y];
f1 = G#0-G#1;
f2 = G#2-G#3;
mixedVolume({f1,f2}) 
\end{verbatim}

% --The volume of the NObody of G should be the number of solutions
% --to a general system drawn from V. 
% --The following checks the general number of solutions to such a system.
% subV = {1+0*x,x*y,x,y} --use this system so we only keep track of the isolated sol'ns
% (solnInstance, sysInstance, mixedVol) = solveInstance(subV)
% #solnInstance
